ProSA: Assessing and Understanding the Prompt Sensitivity of LLMs

Large language models (LLMs) have demonstrated impressive capabilities across various tasks, but their performance is highly sensitive to the prompts utilized. This variability poses challenges for accurate assessment and user satisfaction. Current research frequently overlooks instance-level prompt variations and their implications on subjective evaluations. To address these shortcomings, we introduce ProSA, a framework designed to evaluate and comprehend prompt sensitivity in LLMs. ProSA incorporates a novel sensitivity metric, PromptSensiScore, and leverages decoding confidence to elucidate underlying mechanisms. Our extensive study, spanning multiple tasks, uncovers that prompt sensitivity fluctuates across datasets and models, with larger models exhibiting enhanced robustness. We observe that few-shot examples can alleviate this sensitivity issue, and subjective evaluations are also susceptible to prompt sensitivities, particularly in complex, reasoning-oriented tasks. Furthermore, our findings indicate that higher model confidence correlates with increased prompt robustness. We believe this work will serve as a helpful tool in studying prompt sensitivity of LLMs. The project is released at: https://github.com/open-compass/ProSA .

==> figure/confidence_format.tex <==
\definecolor{lightgray}{gray}{0.95}
\lstdefinestyle{prompt}{
    basicstyle=\ttfamily\fontsize{7pt}{8pt}\selectfont,
    frame=none,
    breaklines=true,
    backgroundcolor=\color{lightgray},
    breakatwhitespace=true,
    breakindent=0pt,
    escapeinside={(*@}{@*)},
    numbers=none,
    numbersep=5pt,
    xleftmargin=3pt,
}
\tcbset{
  aibox/.style={
    % width=220pt,
    top=10pt,
    colback=white,
    colframe=black,
    colbacktitle=black,
    enhanced,
    center,
    % breakable,
    attach boxed title to top left={yshift=-0.1in,xshift=0.15in},
    boxed title style={boxrule=0pt,colframe=white,},
  }
}
\newtcolorbox{AIbox}[2][]{aibox, title=#2,#1}

\begin{figure}[!h]
\begin{AIbox}{Template for Token Probabilities}
{\color{red}\bf User:}"\{Instruction\}\{Input\}"\\
{\color{blue}\bf Assistant:}"The correct answer is the option \_"
\end{AIbox} 
\caption{\textbf{The template for token probabilities.}The template used for calculating model's confidence. Here, the "\{Instruction\}" and "\{Input\}" fields will be replaced by specific instructions and questions. The "\_" represents the content that the model will continue to generate. The final returned result is the probability distribution of the first token for the next tokens prediction task.}
\label{fig:ttp}
\end{figure}

==> table/confidence.tex <==
\begin{table*}[!h]
\centering
\resizebox{0.5\textwidth }{!}{%
\begin{tabular}{l|ccccc}
\toprule
\textbf{Models} & \textbf{1-Option} & \textbf{2-Options} & \textbf{3-Options} & \textbf{4-Options} & \textbf{5-Options} \\
\midrule
\textbf{Mistral-7b} & 0.939 & 0.851 & 0.662 & 0.583 & 0.472 \\
\hline
\textbf{InternLM2-7B} & 0.706 & 0.475 & 0.360 & N\textbackslash A & N\textbackslash A\\
\hline
\textbf{InternLM2-20B} & 0.454 & 0.276 & 0.135 & N\textbackslash A & N\textbackslash A \\
\bottomrule
\end{tabular}
}
\caption{\textbf{The Relationship between Model Confidence and Prompt Sensitivity.} Note that due to variations in model parameter size
and vocabulary size, cross-model confidence comparisons are not meaningful.}
\label{tab:confidence}
\end{table*}

